NADI 2020: The First Nuanced Arabic Dialect Identification Shared Task

We present the results and findings of the First Nuanced Arabic Dialect Identification Shared Task (NADI). This Shared Task includes two subtasks: country-level dialect identification (Subtask 1) and province-level sub-dialect identification (Subtask 2). The data for the shared task covers a total of 100 provinces from 21 Arab countries and are collected from the Twitter domain. As such, NADI is the first shared task to target naturally-occurring fine-grained dialectal text at the sub-country level. A total of 61 teams from 25 countries registered to participate in the tasks, thus reflecting the interest of the community in this area. We received 47 submissions for Subtask 1 from 18 teams and 9 submissions for Subtask 2 from 9 teams.

==> conc.tex <==
\section{Conclusion and Future Work}\label{sec:conc}
We presented an overview of the NADI 2020 shared task. We described the dataset and identified areas of improvement especially related to its collection. We also provided a high-level description of participating teams. The number of submissions to the shared task reflects an interest in the community and calls for further work in the area of Arabic dialect detection, but also more generally Arabic dialect processing. 

In the future, we plan to host a second iteration of the NADI shared task that will use new datasets and pursue a number of novel questions inspired by the issues discovered in this year's task. For example, in addition to DA classification, we will propose {\it MSA regional use  classification} as a subtask. Since MSA is shared across the Arab world, we hypothesize this will be a more challenging task than DA classification. 
We will also encourage teams to experiment with studying the interaction between MSA and DA in novel ways. For example, questions as to the utility of using DA data to improve MSA
regional use  classification systems and vice versa can be investigated exploiting various machine learning methods.

\section*{Acknowledgments}
We gratefully acknowledge the support of the Natural Sciences and Engineering Research Council of Canada (NSERC), the Social Sciences Research Council of Canada (SSHRC), and Compute Canada (\url{www.computecanada.ca}). We thank AbdelRahim Elmadany for assisting with dataset preparation, setting up the Codalab for the shared task, and providing the map in Figure~\ref{fig:province_map}.


==> data.tex <==
\section{Shared Task Datasets}\label{sec:data}
We distributed a single dataset with two sets of labels, one for Subtask~1 and another for Subtask~2. In other words, the same tweet occurs in each of the two subtasks but with different subtask-specific labels.
%(one for country in Subtask~1 and another for province in Subtask~2).
Additionally, we made available an unlabeled dataset for optional use in any of the two subtasks. We now provide more details about both the labeled and unlabeled data.  

\subsection{Data Collection}

We used the Twitter API to crawl data from 100 provinces belonging to 21 Arab countries for 10 months (Jan. to Oct., 2019).\footnote{Although we tried, we could not collect data from Comoros to cover all 22 Arab countries.} Next, we identified users who consistently and \textit{exclusively} tweeted from a single province during the whole 10 month period. We crawled up to 3,200 tweets from each of these users. 

\subsection{Data Sets}

\paragraph{Subtask~1 and Subtask~2 Data} We labeled tweets from each user with the country and province from which the user posted for the whole of the 10 months period, thus exploiting user consistent posting {\it location} as a proxy for {\it  dialect labels}. Note that this labeling method can still have issues as we explain in Section~\ref{subsec:data_issues}. We randomly sampled 30,957 tweets of length 5 words or more from the collection and split them into TRAIN (n=21,000), DEV (n=4,957), and TEST (n=5,000). Although the task is at the tweet level, we sampled the data for each of the TRAIN, DEV, and TEST from a unique set of users (i.e., users are not shared across the 3 splits). We distribute data for the two subtasks directly to participants in the form of actual tweet text (i.e., hydrated content). Tables~\ref{tab:country} and~\ref{tab:data_provinces} show the distribution of tweets across the data splits for both Subtask~1 and Subtask~2, respectively.

\begin{wrapfigure}{r}{0.5\textwidth}
  \begin{center}
  \frame{\includegraphics[width=7cm,height=4.5cm]{images/dis_perc}}
  \end{center}
\caption{Distribution of tweet length in words in NADI labeled data.}
\label{fig:province_map}
\end{wrapfigure}

\paragraph{Unlabeled 10M} ~We also crawled 10 million posts from Arabic Twitter during 2019. We call this dataset UNLABELED 10M and distribute it in the form of tweet IDs along with a script that can be used to crawl the actual tweets. We put no restrictions on using UNLABELED 10M for system development for either of the two subtasks.\footnote{Subtask~1, Subtask~2, and UNLABELED 10M data is available at \url{http://nadi2020.arabic-nlp.net}. More information about the data format can be found in the accompanying README file.} Next, we discuss a number of nuances and issues found in the data.

\subsection{Data Issues}\label{subsec:data_issues}

\paragraph{Location as proxy for dialect.} Our method of using consistent location (i.e., posting from the same location for at least 10 months) as a proxy for assigning dialect labels is useful, but not ideal. Even though this method allows us to collect provably relevant data, as manually verified in a small random sample of users (n=30), it can be error prone since a user with a dialect of one country can be posting from a different country during this whole period of 10 months.  

\paragraph{MSA vs. Dialect.} As we explained in Section~\ref{sec:intro}, Arabic is usually characterized as a diaglossic language with MSA being the `High' variety and DA as the `Low' variety. Arabic users also switch between these two varieties. Most relevant to our work, communication in DA over social media is not devoid of MSA even at a level as short as that of a tweet. This can vary from one dialect to another, but also depending on a range of other factors including the user educational background, career, and the actual goal of the post itself. To illustrate, based on our intuition and occasional observation, users with training in language sciences (education), those in careers such as media or higher education (job), or those trying to reach out to especially older generations or project religious or cultural authority (goal or pragmatic function) will likely use more MSA. Due to the co-existence of MSA and DA in the same tweet, we opted for using all the data we collected from the users for the competition. Alternatively, we could have identified MSA tweets either manually or automatically and removed these. We did not take that step in order to keep the task more challenging since a classifier would need to learn about patterns of MSA-DA mixing to perform well. A model would also need to acquire skills enabling it to tease apart tweets that may be overly or exclusively MSA. To explore the extent of MSA in the dataset, we run an in-house neural MSA-DA model ($acc=89.1\%, F_1=88.6\%$) on it. The model predicts the percentages of MSA data as follows: 49.5\% for TRAIN, 46.6\%for DEV, and 49.7\% for TEST. This distribution needs to be couched with caution, however, since dialectal features can be subtle and mixed with MSA to varying degrees. Upon manual inspection of a random sample of tweets the model labeled as MSA, we identify examples that are fully and verifiably MSA such as \#1 below. In addition, we observe sequences that carry dialectal features. For example \#2 and \#3 below have dialectal words (highlighted in \colorbox{orange!15}{orange}):

\input{misc}

We also observe that the more confident the MSA-DA model is (based on softmax value), the more likely its decision is correct. This suggests we can use a thresholding approach to filter out MSA tweets, should we desire to reduce MSA in the data. We leave further investigation of this issue to the future. %\hl{This shows that a model would need to not only tease apart DA by country or province, but MSA text as well.}

\paragraph{Non-Arabic Text.} Despite efforts to exclusively keep Arabic content, our dataset had a small percentage (2.52\%) of Farsi. While collecting the data, we only kept tweets assigned an Arabic language tag by the Twitter API. However, the API is error prone and hence some non-Arabic was not filtered out. To circumvent this, we only kept tweets that have at least three word written in Arabic script after running an internal normalizer that removes diacritics and reduced repetitions of consecutive characters of $>2$ to only 2, replaced URLs and usernames with the generic strings $URL$ and $@USR$. Even after this step, some Farsi leaked to our data. The reason is that Farsi is written in the same script as Arabic, with only a few differences. \newcite{aliwy:2020:arabic-dialects} manually inspected the NADI TRAIN set and provided a distribution of Farsi tweets over the different countries. We share this distribution in Table~\ref{tab:farsi}.

\begin{wraptable}{r}{0.5\textwidth}
%\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{lrrr}
\hline
\multicolumn{1}{c}{\textbf{Country}} & \multicolumn{1}{c}{\textbf{\# tweet}} & \multicolumn{1}{c}{\textbf{\#  Farsi}} & \multicolumn{1}{c}{\textbf{\% Farsi}} \\ \hline
\textbf{Algeria}                     & 1,491                                              & 5                                       & 0.34                                       \\
%\textbf{Bahrain}                     & 210                                               & 0                                       & 0.00                                       \\
%\textbf{Djibouti}                    & 210                                               & 0                                       & 0.00                                       \\
\textbf{Egypt}                       & 4,473                                              & 2                                       & 0.04                                       \\
\textbf{Iraq}                        & 2,556                                              & 382                                     & 14.95                                      \\
%\textbf{Jordan}                      & 426                                               & 0                                       & 0.00                                       \\
%\textbf{Kuwait}                      & 420                                               & 0                                       & 0.00                                       \\
%\textbf{Lebanon}                     & 639                                               & 0                                       & 0.00                                       \\
%\textbf{Libya}                       & 1,070                                              & 0                                       & 0.00                                       \\
%\textbf{Mauritania}                  & 210                                               & 0                                       & 0.00                                       \\
\textbf{Morocco}                     & 1,070                                              & 1                                       & 0.09                                       \\
\textbf{Oman}                        & 1,098                                              & 26                                      & 2.37                                       \\
%\textbf{Palestine}                   & 420                                               & 0                                       & 0.00                                       \\
%\textbf{Qatar}                       & 234                                               & 0                                       & 0.00                                       \\
\textbf{Saudi Arabia}               & 2,312                                              & 6                                       & 0.26                                       \\
%\textbf{Somalia}                     & 210                                               & 0                                       & 0.00                                       \\
%\textbf{Sudan}                       & 210                                               & 0                                       & 0.00                                       \\
\textbf{Syria}                       & 1,070                                              & 3                                       & 0.28                                       \\
\textbf{Tunisia}                     & 750                                               & 2                                       & 0.27                                       \\
\textbf{UAE}      & 1,070                                              & 7                                       & 0.65                                       \\
\textbf{Yemen}                       & 851                                               & 70                                      & 8.23                                       \\ \hline
\textbf{Total}                     & 21,000                                             & 504                                     & 2.40                                       \\ \hline
\end{tabular}
\caption{Distribution of tweets manually labeled as Farsi in TRAIN. We only provide countries with Farsi tweets, and remove the rest of 21 countries in NADI.}\label{tab:farsi}
\end{wraptable}

==> teams.tex <==
\section{Teams}\label{sec:teams}
We present teams here\dots 
